Enhancing Node Representations for Real-World Complex Networks with Topological Augmentation

Graph augmentation methods play a crucial role in improving the performance and enhancing generalisation capabilities in Graph Neural Networks (GNNs). Existing graph augmentation methods mainly perturb the graph structures, and are usually limited to pairwise node relations. These methods cannot fully address the complexities of real-world large-scale networks, which often involve higher-order node relations beyond only being pairwise. Meanwhile, real-world graph datasets are predominantly modelled as simple graphs, due to the scarcity of data that can be used to form higher-order edges. Therefore, reconfiguring the higher-order edges as an integration into graph augmentation strategies lights up a promising research path to address the aforementioned issues. In this paper, we present Topological Augmentation (TopoAug), a novel graph augmentation method that builds a combinatorial complex from the original graph by constructing virtual hyperedges directly from the raw data. TopoAug then produces auxiliary node features by extracting information from the combinatorial complex, which are used for enhancing GNN performances on downstream tasks. We design three diverse virtual hyperedge construction strategies to accompany the construction of combinatorial complexes: (1) via graph statistics, (2) from multiple data perspectives, and (3) utilising multi-modality. Furthermore, to facilitate TopoAug evaluation, we provide 23 novel real-world graph datasets across various domains including social media, biology, and e-commerce. Our empirical study shows that TopoAug consistently and significantly outperforms GNN baselines and other graph augmentation methods, across a variety of application contexts, which clearly indicates that it can effectively incorporate higher-order node relations into the graph augmentation for real-world complex networks.

==> appendices/data-access.tex <==
\section{Code and Data Accessibility}

The source code and full datasets of SHGB is publicly available at \url{https://anonymous-url/}. %\url{https://zehui127.github.io/hybrid-graph-benchmark/}. 
While the raw dataset in JSON format is hosted at \url{https://anonymous-url/}, %\url{https://zenodo.org/record/7982540}, 
we recommend the users to access the datasets through our Python library \texttt{anonymous-library}, %\texttt{hybrid-graph}, 
which is installable via \texttt{pip}. This would allow the users to read the graphs in the format of PyTorch Geometric \texttt{Data} objects. 



==> appendices/eval-details.tex <==
\section{Experimental Setup} \label{appendix:details}

\subsection{Training Details}

We run all the experiments on NVIDIA A100 PCIe GPUs with 40GB memory (Sulis), NVIDIA V100 NVLink GPUs with 32GB memory (JADE), and NVIDIA V100 SXM2 GPUs with 16GB memory (Cirrus). Adam~\cite{kingma2014method} is used as the optimiser, and CosineAnnealingLR~\cite{gotmare2018closer} is used as the learning rate scheduler for all training. For each experiment, the nodes of the graph dataset are randomly split into training, validation, and test sets with a split ratio of 6:2:2. All models are trained for 500 epochs. For node classification tasks, the negative log likelihood loss (NLLLoss) is used as the loss function. For node regression tasks, the mean square error (MSELoss) is used as the loss function. Training typically takes less than 5 minutes for each experiment, when ED-HNN is not incorporated in the model. Due to the significantly larger architecture of ED-HNN, experiments involving it can take up to 2 hours. 

\subsection{Hyperparameter Settings}

We perform a hyperparameter search for the learning rate and dropout rate, while keeping the hidden dimension of the layers fixed. To ensure fair comparison, all evaluated GNNs (GCN, GAT, GraphSAGE, HyperConv, and ED-HNN) share the same hyperparameter combinations. After hyperparameter searching, we adopt the following hyperparameter selections: learning rate = 0.001, hidden dimension = 64, and dropout rate = 0.5. For the additional hyperparameters of ED-HNN, we closely adhere to the hyperparameter settings specified in the original ED-HNN paper~\cite{Wang2023EDHNN}, and set the number of all inner multi-layer perceptrons (MLPs) within ED-HNN to 2. 
    
